Atomic Representations of Local and Global Chemistry in Complex Alloys

The exceptional properties observed in complex concentrated alloys (CCAs) arise from the interplay between crystalline order and chemical disorder at the atomic scale, complicating a unique determination of properties. In contrast to conventional alloys, CCA properties emerge as distributions due to varying local chemical environments and the specific scale of measurement. Currently there are few ways to quantitatively define, track, and compare local alloy compositions (versus a global label, i.e. equiatomic) contained in a CCA. Molecular dynamics is used here to build descriptive metrics that connect a global alloy composition to the diverse local alloy compositions that define it. A machine-learned interatomic potential for MoNbTaTi is developed and we use these metrics to investigate how property distributions change with excursions in global-local composition space. Short-range order is examined through the lens of local chemistry for the equiatomic composition, demonstrating stark changes in vacancy formation energy with local chemistry evolution.

==> figures_tables/tab1.tex <==

{
%%% These are updated values for averaged ZBL
\begin{table}[b!]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\hline
\textbf{Composition} & \textbf{Property} &  \textbf{DFT}~\cite{startt2022compositional} &  \textbf{SNAP} & \textbf{Error (\%)}\\
\hline
\multirow{Equi.} 
 & $\mathbb{C}_{11}$ [GPa] & 239.6 & 255.3 & 6.6\% \\
 & $\mathbb{C}_{12}$ [GPa] & 129.7 & 139.7 & 7.7\% \\
 & $\mathbb{C}_{44}$ [GPa] & 37.8  & 39.1  & 3.4\% \\
 & $B$ [GPa] & 165.7  & 178.4  & 7.7\% \\
 & $G$ [GPa] & 43.6  & 42.7  & 1.0\% \\
 & $E$ [GPa] & 120.1  & 126.4  & 5.2\% \\
 & $\nu$ & 0.379  & 0.382  & 0.8\% \\
 \hline
 \multirow{Mo 12.5 at.-\%} 
 & $\mathbb{C}_{11}$ [GPa] & 234.3 & 233.8 & 0.2\%  \\
 & $\mathbb{C}_{12}$ [GPa] & 134.6 & 134.3 & 0.2\% \\
 & $\mathbb{C}_{44}$ [GPa] & 35.6  & 36.0  & 1.0\% \\
 & $B$ [GPa] & 167.8  & 167.5  & 0.2\% \\
 & $G$ [GPa] & 40.8  & 40.1  & 0.5\% \\
 & $E$ [GPa] & 113.2 & 113.6  & 0.4\% \\
 & $\nu$ & 0.388  & 0.387  & 0.2\% \\
\hline
 \multirow{Mo 50 at.-\%} 
 & $\mathbb{C}_{11}$ [GPa] & 334.4 & 312.5 & 6.5\%  \\
 & $\mathbb{C}_{12}$ [GPa] & 147.3 & 149.3 & 1.3\% \\
 & $\mathbb{C}_{44}$ [GPa] & 50.331  & 50.0  & 0.6\% \\
 & $B$ [GPa] & 209.7  & 203.7  & 2.9\% \\
 & $G$ [GPa] & 64.7  & 60.9  & 5.8\% \\
 & $E$ [GPa] & 175.9 & 166.2  & 5.5\% \\
 & $\nu$ & 0.360  & 0.364  & 1.1\% \\
\hline
\hline
\end{tabular}
\caption{
Elasticity value comparisons from the MoNbTaTi dataset and the SNAP model for the equiatomic RSS and an example at Mo enriched to 50 at.\%. Each value was averaged over 4 DFT semiquasirandom structure calculations and 5 SNAP calculations. 
}
\label{table:tab1}
\end{table}
}
